On an optimal AFEM for elastoplasticity

In this paper, optimal convergence for an adaptive finite element algorithm for elastoplasticity is considered. To this end, the proposed adaptive algorithm is established within the abstract framework of the axioms of adaptivity [Comput. Math. Appl., 67(6) (2014), 1195-1253], which provides a specific proceeding to prove the optimal convergence of the scheme. The proceeding is based on verifying four axioms, which ensure the optimal convergence. The verification is done by using results from [Numer. Math., 132(1) (2016), 131-154], which presents an alternative approach to optimality without explicitly relying on the axioms.

==> misc.tex <==
The study of adaptive finite element methods regarding partial differential equations has been of interest for many years. Convergence of such adaptive finite element methods was first discussed in \cite{Bubuska} and proven in \cite{Doerfler} and has been further studied in e.g. \cite{BDVNVB,DorflerWilde, Morin,DataoscConvergence}. Optimal convergence of adaptive finite element methods has been verified in several cases, e.g. \cite{NochettoQuasiOptimal, FeischlOptimal,StevensonStokes,StevensonOptimality}. In \cite{Axioms} an approach for the verification of optimal convergence was outlined. The results of \cite{Axioms} showed for the standard loop of
\begin{center}{\textbf{Solve} \(\rightarrow\) \textbf{Estimate} \(\rightarrow\) \textbf{Mark} \(\rightarrow\) \textbf{Refine}}\end{center}
that if an adaptive finite element method satisfies a set of four axioms, optimal convergence of that method is guaranteed. These four axioms of adaptivity are stability (A1), reduction property (A2), general quasi-orthogonality (A3) and discrete reliability (A4).\\
In mechanical engineering, adaptive finite element methods are used to solve partial differential equations arising from certain physical processes. One such process is the behaviour of elastoplastic material under the influence of stress. These type of materials behave elastically until a certain threshold of stress is exceeded. Then these material undergo plastic deformation. The model of elastoplasticity is described through a variational inequality of the second kind, where a non-differentiable term introduces non-linear behaviour. An analysis of this model can be found in e.g. \cite{CarstensenDiscrete,CarstensenReliability,SchroederWiedemann}. Concerning optimal convergence, the work of \cite{ElastoAFEM} discussed an adaptive finite element method for elastoplasticity and proved its optimality independent of the results in \cite{Axioms}\\
The aim of this paper is to prove that the adaptive finite element method for elastoplasticity described in \cite{ElastoAFEM} satisfies the axioms of adaptivity of \cite{Axioms} and  to derive optimal convergence through these axioms. Furthermore, this paper presents a comparison of the two proof methodologies, discussing similarities and differences between the two approaches.\\
To that end, we verify that the error measure and error estimation satisfy the necessary requirement. Also, we confirm that the refinement strategy of newest vertex bisection - generalized to dimensions equal or higher than two as in \cite{Maubach, StevensonNVB, Traxler} -  fulfil the required properties. 
Afterwards, we apply the results from \cite{ElastoAFEM} to show that the axioms of adaptivity hold.\\
With the optimal convergence established by use of the axiom of adaptivity, we then compare that methodology with the approach of \cite{ElastoAFEM}. We begin with the proof of plain convergence. This comparison highlights two lemmas of \cite{ElastoAFEM}, which act as counterparts to the axioms stability (A1) and reduction property (A2). Additionally, it shows how reliability is treated differently in both papers: as an independent result in \cite{ElastoAFEM} and as a consequence of the discrete reliability (A4) in \cite{Axioms}.\\
In the course of the comparison, we also verify how the efficiency of the error estimator implies the equivalence of the two definitions of optimal convergence. Then, when examining the two proofs of optimal convergence side by side, it becomes clear that they both follow the same structure. However, we emphasize one key difference: the use of efficiency in \cite{ElastoAFEM}. While other arguments remain similar in both proofs, the use of efficiency stands out as the proof of optimality of \cite{Axioms} does not need the efficiency of the error estimator at any point. This shows a clear advantage of the approach of \cite{Axioms}, which remains applicable even if the error estimator is not efficient, whereas the method of \cite{ElastoAFEM} depends on the efficiency of the estimator.\\
The paper is organized as follows. In section \ref{Section2 Model of Elasto} we introduce the one quasi-static time step of the primal problem of elastoplasticity with isotropic and linear kinematic hardening and derive its weak formulation as a variational inequality. In section~\ref{Section3 Discretization} we discuss the discretization with adaptive finite elements. Section~\ref{Section4 An optimal AFEM} is devoted to the proof of the axioms of adaptivity. We first introduce some preliminaries of \cite{ElastoAFEM}, before we prove that the axioms (A1) Stability on non-refined element domains, (A2) Reduction property on refined element domains, (A3) General quasi-orthogonality, (A4) Discrete reliability hold. At the end, we briefly discuss how optimal convergence follows from that. In the last section, the two proofs are compared. We discuss the plain convergence and conclude with optimality and optimal convergence.\\
This paper uses standard notation of Lebesgue and Sobolev spaces and denotes  the \(L^2\) inner product by \((\cdot,\cdot)_{L^2}\). Throughout this paper, \(X\lesssim Y\) abbreviates \(X\leq C\:Y\) for some positive constant C.
